YM2413-MDB: A Multi-Instrumental FM Video Game Music Dataset with Emotion Annotations

Existing multi-instrumental datasets tend to be biased toward pop and classical music. In addition, they generally lack high-level annotations such as emotion tags. In this paper, we propose YM2413-MDB, an 80s FM video game music dataset with multi-label emotion annotations. It includes 669 audio and MIDI files of music from Sega and MSX PC games in the 80s using YM2413, a programmable sound generator based on FM. The collected game music is arranged with a subset of 15 monophonic instruments and one drum instrument. They were converted from binary commands of the YM2413 sound chip. Each song was labeled with 19 emotion tags by two annotators and validated by three verifiers to obtain refined tags. We provide the baseline models and results for emotion recognition and emotion-conditioned symbolic music generation using YM2413-MDB.

==> dummy_table.tex <==
% \begin{table*}[]
% \renewcommand{\arraystretch}{1.2} % for table margin
% \begin{center}
% \begin{tabular}{c|cc|cc|c}

% \toprule
% \textbf{}                                                                                       & LMD                                                                                   & NES-MDB                                                                                                                                                     & VGMIDI                    & EMOPIA           & YM2413-MDB (ours)                                                                                                                                     \\ \midrule
% \# Instruments                                                                                  & 128                                                                                                           & 4                                                                                                                                                           & 1                         & 1                & 17                                                                                                                                                    \\
% \# Avg Tracks                                                                                   & 8.8 / no limit                                                                                                & 2.8 / max 4                                                                                                                                                 & 1                         & 1                & 7.2 / max 9                                                                                                                                           \\
% \# Songs                                                                                        & 178K                                                                                                          & 5.2K                                                                                                                                                        & 200                       & 1078             & 655                                                                                                                                                   \\
% \begin{tabular}[c]{@{}c@{}}Total Length\end{tabular}                                                                          & 9K hours                                                                                                            & 46.1 hours                                                                                                                                                      &                           & 11 hours              & 10.6 hours                                                                                                                                                 \\
% Music Style                                                                                     &\begin{tabular}[c]{@{}c@{}}General \\ (Karaoke)\end{tabular}                                                                                              & \begin{tabular}[c]{@{}c@{}}Game music \\ (early 80s)\end{tabular}                                                                                                                                      & \begin{tabular}[c]{@{}c@{}}Piano-arranged\\ game music\end{tabular} & Pop piano music  & \begin{tabular}[c]{@{}c@{}}Game music \\ (late 80s)\end{tabular}                                                                                                                                 \\
% Data Collection                                                       & Crawling                                                                    & \begin{tabular}[c]{@{}c@{}}Sound chip emulation\\ (oscillator, filter)\end{tabular} & Crawling & Crawling & \begin{tabular}[c]{@{}c@{}}Sound chip emulation\\ (FM synthesis)\end{tabular} \\
% Label Type                                                                                      & None                                                                                                          & None                                                                                                                                                        & Valence                   & Russell's 4Q     & 19 Emotion related tags                                                                                                                  \\ \bottomrule
% \end{tabular}
% \end{center}
% \caption[General Dataset Statistics]{Comparison with existing multi-instrumental or emotion-labeled datasets and the proposed YM2413-MDB}
% \end{table*}



%%%%%%% TABLE %%%%%%%
% \begin{table*}[htp!]
% \begin{center}
% \begin{tabular}{l|llllll|rrrrr}
% \toprule
% \multicolumn{1}{c|}{\multirow{}{}{\textbf{Model}}} & \multicolumn{6}{c|}{\textbf{Objective metrics}}  & \multicolumn{5}{c}{\textbf{Subjective metrics}}                                                                            \\ \cline{2-12} 
% \multicolumn{1}{c|}{}                                & PCH & NLH & \multicolumn{1}{l|}{IH} & 4Q & A & V & \multicolumn{1}{c}{ST} & \multicolumn{1}{c}{HR} & \multicolumn{1}{c}{RH} & \multicolumn{1}{c}{OQ} & \multicolumn{1}{c}{LO} \\ \midrule
% YM2413-MDB (i.e. real data)                          &     &     & \multicolumn{1}{l|}{}   &    &   &   &                        &                        &                        &                        &                        \\ \midrule
% GPT2                                                 &     &     & \multicolumn{1}{l|}{}   &    &   &   &                        &                        &                        &                        &                        \\
% GPT2 w/ pre-training                                 &     &     & \multicolumn{1}{l|}{}   &    &   &   &                        &                        &                        &                        &                        \\ \bottomrule
% \end{tabular}
% \end{center}
% \caption[General Dataset Statistics]{Comparison with existing multi-instrumental or emotion-labeled datasets and the proposed YM2413-MDB}
% \end{table*}


%%%%%%% TABLE %%%%%%%
% \begin{figure}[htp!]
%  \centerline{
%  \includegraphics[width=\columnwidth]{figs/emotion tag cooc.png}}
%  \caption{Co-occurrence of emotion tags. Each column is normalized by the frequency of each tag.}
%  \label{fig:emotion tag cooc}
% \end{figure}

% \begin{figure}[htp!]
%  \centerline{
%  \includegraphics[width=\columnwidth]{figs/frequency distribution of tags7x7.png}}
%  \caption{Frequency distribution of emotion tags after verification.}
%  \label{fig:emotion tag frequency}
% \end{figure}


% \begin{figure*}[htp!]
%      \centering
%      \begin{subfigure}[b]{0.47\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/note density.jpg}
%          \caption{Note density}
%          \label{fig:cls note density}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.47\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/note length.jpg}
%          \caption{Note length}
%          \label{fig:cls note length}
%      \end{subfigure}
%         \caption{Violin plots of the distribution in note density and note length for different top tag classes}
%         \label{fig:cls note distribution}
% \end{figure*}


% \begin{figure}[]
%  \centerline{
%  \includegraphics[width=\columnwidth,height=5cm]{figs/mode distribution.jpg}}
%  \caption{Key distribution of different top tag classes}
%  \label{fig:key distribution cls}
% \end{figure}


==> dummy_text.tex <==
% \section{Dataset Analysis}
% Here, we conducted case studies with the characteristics of the YM2413-MDB. We found two composition patterns, such as unison playing and simulated reverb using delay. These patterns are unique because they are only observed in early video game music due to the limitation of technology at that time. 
% \subsection{Unison Playing}
% Unlike other datasets, such as Lakh or NES-MDB, there is a pattern of playing the same melody with more than two instruments in YM2413-MDB. These patterns are used to make a rich sound by overlapping the same voices of FM instrument. We call this pattern Unison playing since in most of cases the instruments are playing exactly the same voices. As these patterns are also observed as the same voices with not only the same but also different instruments, the composers could make more diverse timbre of sounds by using this technique.

% \subsection{Delay and Reverb Effects}
% Another composition pattern that can be observed in the YM2413-MDB is implemented-reverb using delay. This pattern is also observed in NES music \cite{gutierrez2016programmed}, to express the reverb as using the delayed same voice. Among composition techniques of NES music that were mentioned in \cite{gutierrez2016programmed}, this is the only pattern that we found in the YM2413-MDB. This shows the improvement of the hardware sound chip and changed the composition patterns: YM2413 sound chip has more capacity to express the note of instruments(nine) to play at once than NES(four).

% To evaluate the generated game music, we conducted a human evaluation as qualitative evaluation. 
% \subsubsection{Stimuli}
% For evaluation, nine music samples were used: we selected three generated music each from train splits of YM2413-MDB, a pre-trained model using Lakh dataset, and fine-tuned model using YM2413-MDB. Since we evaluated the looping, we made 16-bar samples by repeating the 8-bar generated samples twice. For the samples from the dataset, we selected samples that have a repetition of 8-bar. After that, we rendered all samples using VST2413 \footnote{http://www.keijiro.tokyo/vst2413/}, which is a software synthesizer that implemented the FM-synthesized timbre of YM2413 instruments.

% \section{Results and Discussion}
% In this section, we explored the generated music using this new dataset. Furthermore, we evaluated the generated music in objective and subjective ways. We compared generated music samples with the Lakh dataset, YM2413-MDB, and as well as samples from Lakh pre-trained model.

% \subsection{Objective Evaluation}
% We investigated whether the fine-tuning stage can help the deep learning model to capture the musical features of the 80s game such that the model can generate music similar to the 80s game. The result of this experiment is shown in Table ~\ref{objective-tab}. Overall, we observed lower KLD and higher OA values for the training dataset with YM2413-MDB fine-tune condition than Lakh pre-train condition. Low KLD and high OA imply two distributions are similar. For the pitch histogram feature, KLD was lower for Lakh pre-train condition than for the YM2413-MDB fine-tune condition. However, as \cite{yang2020evaluation} discussed, both KLD and OA should be considered because each KLD and OA cannot fully express the distribution comparison when used alone: high KLD with high OA means the distribution shape is not similar, but the overall mean and std are similar. From this result, we can infer that the fine-tuned model generates samples similar to the YM2413-MDB than Lakh pre-train model, which also confirms that the fine-tuning stage was valid.

% \subsection{Subjective Evaluation}
% To validate the generated result, we did a human evaluation of the listening test as a subjective evaluation. Table ~\ref{subjective-tab} shows the result of subjective evaluation. Overall, the music from the YM2413-MDB had the highest score of all metrics. Also, from the result, we found that the average of all evaluation metrics of generated music by the YM2413-MDB fine-tuned model was 3.56, which score is higher than samples from Lakh pre-trained model. It is worth noting that the participants did agree that generated music from the YM2413-MDB fine-tuned model is game music than the Lakh-pre-trained model. Also, samples from YM2413-MDB fine-tuned model received higher scores for looping and structure than the Lakh pre-trained dataset. This infers the model learned a feature of looping from the game dataset. 

% However, the samples for comparison were small thereby it cannot show the diversity of generated music from models. Since another characteristic of game music is a repeated theme with different BGM, the diversity of generated music should also be assessed. Therefore, further examination of generated samples by comparing each model with how many different samples can be generated when the same prompt such as 4 bar template or a melody theme is given.

% Since there are few high-level annotated datasets, most of these studies controlled low-level features such as pitch, rhythm density \cite{chen2020musicsketchnet, tan2020musicfadernet, wu2021musemorphose}, and polyphony \cite{wu2021musemorphose} or bar \cite{jiang2020transformervae}, which can be directly extracted from the dataset. 

% The most widespread multi-instrumental symbolic music dataset is the Lakh MIDI dataset(LMD) \cite{raffel2016learning}. While it is the only large-scale MIDI dataset, the arrangement style and the transcribed quality are not consistent within the dataset. Another available dataset is Nintendo Entertainment System Music Database (NES-MDB), the early 80’s Nintendo Game Music Dataset \cite{donahue2018nes}. All music in NES-MDB has four monophonic instruments because of the strong technical constraint of NES’s Audio Processing Unit (APU). Due to such strong constraints and the context of chiptune game music, NES-MDB has a stylistic consistency that can be captured by deep learning models \cite{donahue2019lakhnes}. Another characteristic of NES-MDB is expressiveness, in which the ticks of the MIDI file are set identically with the APU's clock to preserve the expressiveness of the original sound. However, such stylistic consistency and expressiveness of NES-MDB make it hard to apply further musical analysis (music genre, instrument, tonality) or utilize other musical information (chord, bar, beat) while generating music. Neither of these datasets has any high-level annotation.	

% 2021 ISMIR controllable music generation paper 추가하기
% emopia에 적혀 있는 다른 사전 연구들 추가하기
% Another issue of music generation is controllability. Most of current music generation studies let the system generate music from scratch without any interaction with the user. When we consider the practical usage of the music generation system, music generation research with controllable parameters is needed. However, 



% Before the main verification experiment, we did the pilot experiment. Through the pilot experiment, we could see that even the meaning of each word differ for each individual even though it is same word. Therefore, when verification experiment, 



% 5 had an intermediate level of music theory knowledge; they knew non-diatonic chords such as secondary dominant and subdominant minor. Eleven have music composition experience(8 had more than three years of music composition, one music composition major).

% Game music is an important element of the game that shapes the overall atmosphere of a game and also greatly affects the player's game experience. \cite{prechtl2016adaptive, mauthes2018vgm} In general, game music is played by loading pre-composed music according to the game situation \cite{prechtl2016adaptive}. In this case, as the number of game maps and situations increases and characters become more diverse, a larger amount of music must be produced.  Therefore, there is an industrial demand for creating game music for games more easily and diversely. In addition, since game music is made for a specific place or situation such as a village, forest, victory, and defeat, the composition intention is relatively clear. This characteristic of game music makes it relatively easier to define high-level conditions and is suitable for conditional music generation.

% However, despite its significance in terms of industry and research, there is currently a lack of research data to generate game music. Datasets currently available for research include NES-MDB \cite{donahue2018nes}, a Nintendo game music dataset in the early 1980s. However, due to hardware limitations, all music in NES-MDB contains up to four instruments, and the resulting unique composition pattern \cite{gutierrez2016programmed, gutierrez2018impact} has the disadvantage of not being able to distinguish and model the roles of each instrument, thereby making it difficult to expand research beyond 8-bit music. Therefore, a game music dataset that expresses a wider variety of music styles and tones is needed. 

% This template includes all the information about formatting manuscripts for the ISMIR \conferenceyear\ Conference.
% Please follow these guidelines to give the final proceedings a uniform look.
% Most of the required formatting is achieved automatically by using the supplied
% style file (\LaTeX) or template (Word).
% If you have any questions, please contact the Program Committee (\texttt{ismir\conferenceyear-papers@ismir.net}).
% This template can be downloaded from the ISMIR \conferenceyear\ web site (\texttt{http://ismir\conferenceyear.ismir.net}).
%

% In Fig ~\ref{fig:violin plot cls} and Fig ~\ref{fig:key distribution cls}, we analyzed the YM2413-MDB with the five top tag emotion: tense, cheerful, touching, bizarre, and depressed. 
% Due to the imbalanced distribution of top tags, we analyzed songs which contain five top tags: tense, cheerful, touching, bizarre, and depressed.

% Ticks per beat was re-calculated using the median of estimated tempos. After tempo calculation, we found that most of the music in the YM2413-MDB has single, fixed BPM of 150.

We split the whole dataset into ten subsets, and each verifier (in total ten verifiers) was assigned to three of them. 
 As a result, each piece was verified by three verifiers. 
